Masked Audio Text Encoders are Effective Multi-Modal Rescorers

Masked Language Models (MLMs) have proven to be effective for second-pass rescoring in Automatic Speech Recognition (ASR) systems. In this work, we propose Masked Audio Text Encoder (MATE), a multi-modal masked language model rescorer which incorporates acoustic representations into the input space of MLM. We adopt contrastive learning for effectively aligning the modalities by learning shared representations. We show that using a multi-modal rescorer is beneficial for domain generalization of the ASR system when target domain data is unavailable. MATE reduces word error rate (WER) by 4%-16% on in-domain, and 3%-7% on out-of-domain datasets, over the text-only baseline. Additionally, with very limited amount of training data (0.8 hours), MATE achieves a WER reduction of 8%-23% over the first-pass baseline.

==> section/Intro-bckup.tex <==

\section{Introduction}
% part 1: Introduce the importance of incorporating LM to E2E ASR

% The recent advances in End-to-End (E2E) Automatic Speech Recognition (ASR) systems \cite{pmlr-v32-graves14, deepspeech, e2e-att-fist-res, Miao2015EESENES, e2e-att-lv, LAS, RNNT, transformer-transducer, conformer} have greatly surpassed the performance of Hybrid ASR Systems \cite{hybrid-dnn, hybrid-survey}. Despite their effectiveness and efficiency, E2E ASR systems heavily rely on a large amount of paired audio-text data, making it difficult to integrate an external Language Model (LM) during training, as hybrid ASR systems can.

%End-to-end (E2E) automatic speech recognition (ASR) system \cite{pmlr-v32-graves14, deepspeech, e2e-att-fist-res, Miao2015EESENES, e2e-att-lv, LAS, RNNT, transformer-transducer, conformer} has greatly improved the performance over the recent past, outperforming hybrid ASR system \cite{hybrid-dnn, hybrid-survey} that decouples acoustic model and language model training. However, despite its effectiveness and the efficiency, E2E ASR system relies heavily on large amount of paired audio-text data, thus there is no trivial way of integrating external language model (LM) during training as hybrid ASR system does. %  By contrast, hybrid ASR decouples acoustic model and language model training, enabling easy incorporation of any independent language model. 

% part 2: Introduce 2nd pass rescoring
Performance of automatic speech recognition (ASR) systems has been traditionally improved using external Language Models (LMs) during inference time %via first-pass language model fusion \cite{zhao19d_shallow_fusion, density_ratio_19_lm_fusion, sriram18_code_fusion} and 
via second-pass rescoring \cite{delibration_neurips17, audio_att_2020,delibration_e2e_asr_20}. %Second-pass rescoring typically relies solely on language models to rerank the first-pass n-best hypotheses\cite{Schwartz1991nbest}.
%Mainstream approaches to improve E2E ASR performance using external LMs during inference time include first-pass language model fusion \cite{zhao19d_shallow_fusion, density_ratio_19_lm_fusion, sriram18_code_fusion} and second-pass rescoring (\todo{CITE}), both can be combined to yield even better results. Therefore, second-pass rescoring has become a standard component in industrial ASR system. Second-pass rescoring strategies typically rely solely on language models to rerank the first-pass n-best hypotheses. (\todo{cite some 2nd pass rescoring papers}) However, recent research work \cite{sainath19_interspeech} (\todo{ADD MORE CITE}) also shows the potential of taking acoustic information as additional input.  % TODO: add more typical second pass mainstream approaches 
% Transformer-based pre-trained LM
In the recent studies, transformer-based pre-trained large language models (LLMs) have shown promising results when used as second-pass rescorers.  According to \cite{rescoreBERT, salazar-etal-2020-masked, llm_22interspeech}, 
BERT\cite{devlin-etal-2019-bert}, a deep bidirectional Transformer \cite{transformer} trained on a Masked Language Model (MLM) loss, performs better than its unidirectional counterparts such as GPT \cite{gpt1} on second-pass rescoring task. They have shown that LLM’s knowledge is most helpful for improving ASR on content words and removing incorrect rare words. 

However, these models have been trained on a wide variety of text data, which may not be representative of the specific domain of interest, leading to poor generalization ability. Also, there is also a risk of overfitting, particularly when using these models for second-pass rescoring. The models may be trained on a specific task or dataset, and may not generalize well to new, unseen data. Another limitation of using large language models for ASR rescoring is their lack of robustness against noise and other types of distortions. These models are typically trained on clean, high-quality speech data, and may not be well-suited for handling the real-world variability and noise present in many speech recognition tasks. This can result in poor performance in noisy or adverse environments.
% \cite{salazar-etal-2020-masked} 
% because of its bidirectional nature.

% % Introduce Multi-modality
% \textbf{Multi-modality Learning} has been an important research area in recent years. The advantages of multi-modality learning over single-modality learning include: 

% 2-nd pass rescoring with multi-source
In response to LLM's failure in domain generalization and robustness, recent research \cite{sainath19_interspeech, audio_att_2020, delibration_e2e_asr_20} has demonstrated the potential of incorporating acoustic information as an additional input for second-pass rescoring. \cite{sainath19_interspeech} proposes a two-pass rescoring method, using Listen, Attend, and Spell (LAS) \cite{LAS} decoder as the second-pass rescorer, by passing the output from a shared LAS and RNN-T \cite{RNNT} encoder as an additional source to the rescorer. This two-pass rescoring method alleviates the generalization issue.
However, it suffers from two main drawbacks: (i) it cannot be trained on unlabeled audio data, (ii) it is inflexible due to its deep integration with the first-pass.

% \textbf{SSL Speech Representations} \cite{Baevski2019vqwav2vecSL, zheng-etal-2021-wav-bert,wav2vec2.0, hubert, Chen2021WavLMLS} leverage large amount of untranscribed speech data, reducing data labeling burden, and bring significant performance improvement on ASR task, especially under low-resource scenarios. The most recent studies \cite{hubert, wav2vec2.0, Chen2021WavLMLS}, motivated by the masked language model loss in NLP, design losses to predict discrete targets of the masked regions. 
% Introduce our novelty and compare with previous work
% Inspired by previous research work, we design a second-pass rescoring architecture which attends to both audio and text modalities. In our work, however, instead of directly using shared acoustic features of the first-pass model, we propose to leverage a pre-trained SSL speech representation model as the acoustic feature extractor. Whereas the acoustic feature extractor (the shared encoder) in LAS rescoring method only benefits from the paired audio-text data, the integration of SSL speech representation model enables taking advantage of the large-scale untranscribed speech data.
In this paper, we propose \mymethod, a multi-modal MLM rescorer that generalizes well to unseen domains. It combines strengths of both pretrained LM rescoring and two-pass rescoring. Our main contributions are summarized as follows:
(1) we introduce the first attempt to integrate a pre-trained self-supervised learning (SSL) speech representation model \cite{Baevski2019vqwav2vecSL, zheng-etal-2021-wav-bert,wav2vec2.0, hubert, Chen2021WavLMLS} into second-pass rescoring. We claims that the integration enables leveraging large-scale unlabeled audio data. 
(2) we prove the effectiveness of adding contrastive loss explicitly in improving the generalization ability of second-pass rescoring.
% \mymethod is fully decoupled from the first-pass ASR, making it agnostic to ASR system architecture, training mechanism and internal features. This addresses the limitations of two-pass rescoring methods while achieving better performance.
(3) furthermore, we demonstrate that content words accuracy (evaluated by CWER) can be further improved on top of LLMs by multi-modal learning.



% \textbf{[Contributions/Novelties]} To the best of our knowledge, this work is the first to

% 1. Propose a multi-modal rescoring framework using masked language models like BERT on top of an encapsulated ASR system: the rescoring approach is agnostic to ASR architecture, training mechanism and internal features. [On the contrary to cascaded two pass systems (https://arxiv.org/pdf/1908.10992.pdf)]

% 2. Incorporate contrastive learning to encourage the rescoring model to learn the features of two distinct modalities - text and audio. 

% Empirical results show the multimodal rescoring approach in out-of-domain evaluation sets can generally achieve on par with in-domain setting. This demonstrates our approach has potential for generalization, without large amount of in-domain training data. 


% (Related Work)
% 0.25 page
% \paragraph{Second Pass rescoring for ASR systems}
% LAS rescoring
% MLM rescoring

% \paragraph{Pre-trained Language Models with Dynamic Prefix}



==> table/ablation.tex <==
\begin{table*}[t!]

\tiny
\centering

% \vspace{0.4em}

\begin{tabular}{l|cccccclc|cccccc}
\hline
\textbf{}                                                                     & \multicolumn{8}{c|}{\textbf{In-domain}}                                                                                                                                                      & \multicolumn{6}{c}{\textbf{Out-of-domain}}                                                                  \\
                                                                              & \multicolumn{2}{c}{\textbf{MTDialogue (seen)}} & \multicolumn{2}{c}{\textbf{LS test-clean}} & \multicolumn{2}{c}{\textbf{LS test-other}} & \multicolumn{2}{c|}{\textbf{Voxpopuli}}           & \multicolumn{2}{c}{\textbf{WSJ}} & \multicolumn{2}{c}{\textbf{ConvAI}} & \multicolumn{2}{c}{\textbf{SLURP}} \\
\textbf{}                                                                     & \textbf{WER}          & \textbf{RWERR}         & \textbf{WER}        & \textbf{RWERR}       & \textbf{WER}         & \textbf{RWERR}      & \multicolumn{1}{c}{\textbf{WER}} & \textbf{RWERR} & \textbf{WER}   & \textbf{RWERR}  & \textbf{WER}     & \textbf{RWERR}   & \textbf{WER}     & \textbf{RWERR}  \\ \hline
No rescoring                                                                  & 9.47                  & -                      & 6.48                & -                    & 12.04                & -                   & 11.06                            & -              & 8.16           & -               & 5.89             & -                & 24.91            & -               \\
BERT w/ FT                                                                  & 9.05                  & 0.0\%                  & 5.50                & 0.0\%                & 10.70                & 0.0\%               & 10.33                            & 0.0\%          & 6.46           & 0.0\%           & 5.38             & 0.0\%            & 24.48            & 0.0\%           \\
\hline
Frozen-BERT                                                                   & 9.21                  & -1.8\%                 & 5.57                & -1.3\%               & 10.82                & -1.1\%              & 10.37                            & -0.4\%         & 6.55           & -1.4\%          & 5.42             & -0.7\%           & 24.39            & 0.4\%           \\
WavLM-adapter &  9.15 & -1.1\% & 5.58 & -1.5\% & 10.81 & -1.0\% & 10.23 & 1.0\% & 6.52 & -0.9\% & 5.47 & -1.7\% & 24.56 & -0.3\% \\
Enc-adapter & 9.19 & -1.5\% & 5.56 & -1.1\% & 10.79 & -0.8\% & 10.09 &  2.3\% & 6.43 & 0.5\%  & 5.42 & -0.7\% & 24.34 & 0.6\% \\
\hline
\mymethod-NA                                                                 & 9.05                  & 0.0\%                  & 5.55                & -0.9\%               & 10.75                & -0.5\%              & 10.34                            & -0.1\%         & 6.49           & -0.5\%          & 5.40             & -0.4\%           & 24.46            & 0.1\%           \\
\mymethod-MSE                                                        & \textbf{7.49}         & \textbf{17.2\%}        & 5.22                & 5.1\%                & 10.31                & 3.6\%               & 10.10                            & 2.2\%          & 6.10           & 5.6\%           & \textbf{5.07}    & \textbf{5.8\%}   & 23.84            & 2.6\%           \\
\mymethod & 7.64                  & 15.6\%                 & \textbf{5.16}       & \textbf{6.2\%}       & \textbf{10.30}       & \textbf{3.7\%}      & \textbf{9.91}                    & \textbf{4.1\%} & \textbf{6.01}  & \textbf{7.0\%}  & 5.10             & 5.2\%            & \textbf{23.77}   & \textbf{2.9\%}  \\ \hline
% \begin{tabular}[c]{@{}l@{}}\mymethod \\ (Full tuning + CTR loss)\end{tabular} & 7.64                  & 15.6\%                 & \textbf{5.16}       & \textbf{6.2\%}       & \textbf{10.30}       & \textbf{3.7\%}      & \textbf{9.91}                    & \textbf{4.1\%} & \textbf{6.01}  & \textbf{7.0\%}  & 5.10             & 5.2\%            & \textbf{23.77}   & \textbf{2.9\%}  \\ \hline
\end{tabular}


\caption{Ablation study is divided into two parts. Part 1 includes parameter-efficient training experiments. \textbf{Frozen-BERT}: all parameters are trainable except BERT (including text embedding), no contrastive loss was added; \textbf{WavLM-adapter}: add bottleneck adapter to speech encoder (WavLM) and do adapter-tuning on WavLM, all other parameters are trainable. \textbf{Enc-adapter}: do adapter-tuning on BERT encoder, all other parameters are trainable. Part 2 investigates the role of explicit alignment loss. \textbf{\mymethod-NA}: same architecture as \mymethod but no additional explicit alignment loss; \textbf{\mymethod-MSE}: same architecture as \mymethod and replace contrastive loss with MSE loss.}

\label{table_ablation}
\end{table*}

==> table/main_bck.tex <==
\begin{table*}[t!]
\tiny
\centering
\vspace{0.1em}
\begin{tabular}{l|cccccccc|cccccc}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{}}} & \multicolumn{8}{c|}{\textbf{In-domain}}                                                                                                                                            & \multicolumn{6}{c}{\textbf{Out-of-domain}}                                                                  \\
\multicolumn{1}{c|}{}                           & \multicolumn{2}{c}{\textbf{MTDialogue (seen)}} & \multicolumn{2}{c}{\textbf{LS test-clean}} & \multicolumn{2}{c}{\textbf{LS test-other}} & \multicolumn{2}{c|}{\textbf{Voxpopuli}} & \multicolumn{2}{c}{\textbf{WSJ}} & \multicolumn{2}{c}{\textbf{ConvAI}} & \multicolumn{2}{c}{\textbf{SLURP}} \\
\multicolumn{1}{c|}{}                           & \textbf{WER}          & \textbf{CWER}          & \textbf{WER}         & \textbf{CWER}       & \textbf{WER}         & \textbf{CWER}       & \textbf{WER}       & \textbf{CWER}      & \textbf{WER}    & \textbf{CWER}  & \textbf{WER}     & \textbf{CWER}    & \textbf{WER}     & \textbf{CWER}   \\ \hline
No rescoring                                    & 9.47                  & 14.63                  & 6.75                 & 8.07                & 11.98                & 15.61               & 11.06              & 10.33              & 8.16            & 8.75           & 5.89             & 9.00             & 24.91            & 29.53           \\
GPT2                                            & 9.32                  & 14.37                  & 6.45                 & 7.78                & 11.70                & 15.11               & 10.72              & 9.94               & 7.64            & 8.40           & 5.76             & 8.66             & 24.91            & 29.53           \\
Multi-modal-GPT2                                        & 9.24                  & 14.17                  & 6.35                 & 7.69                & 11.54                & 14.93               & 10.56              & 9.83               & 7.55            & 8.20           & 5.69             & 8.59             & 24.89            & 29.40           \\
BERT w/ FT                                       & 9.05                  & 13.88                  & 5.50                 & 7.20                & 10.70                & 14.45               & 10.33              & 9.96               & 6.46            & 8.20           & 5.38             & 8.37             & 24.48            & 29.27           \\
\mymethod                                       & \textbf{7.64}         & \textbf{11.70}         & \textbf{5.16}        & \textbf{6.84}       & \textbf{10.30}       & \textbf{13.81}      & \textbf{9.91}      & \textbf{9.47}      & \textbf{6.01}   & \textbf{7.46}  & \textbf{5.10}    & \textbf{7.91}    & \textbf{23.77}   & \textbf{28.14}  \\ \hline
\end{tabular}
\caption{Performance measured by WER $\downarrow$ and CWER $\downarrow$. \mymethod consistently outperforms both text-only (BERT w/ FT) and multi-modal (Multi-modal-GPT2) rescoring baselines across both in-domain and out-of-domain evaluation sets.}

\label{table_main}
\end{table*}
